On the Security of Key Extraction from Measuring Physical Quantities

Key extraction via measuring a physical quantity is a class of information theoretic key exchange protocols that rely on the physical characteristics of the communication channel to enable the computation of a shared key by two (or more) parties that share no prior secret information. The key is supposed to be information theoretically hidden to an eavesdropper. Despite the recent surge of research activity in the area, concrete claims about the security of the protocols typically rely on channel abstractions that are not fully experimentally substantiated. In this work, we propose a novel methodology for the {\em experimental} security analysis of these protocols. The crux of our methodology is a falsifiable channel abstraction that is accompanied by an efficient experimental approximation algorithm of the {\em conditional min-entropy} available to the two parties given the view of the eavesdropper. We focus on the signal strength between two wirelessly communicating transceivers as the measured quantity and we use an experimental setup to compute the conditional min-entropy of the channel given the view of the attacker which we find to be linearly increasing. Armed with this understanding of the channel, we showcase the methodology by providing a general protocol for key extraction in this setting that is shown to be secure for a concrete parameter selection. In this way we provide a first comprehensively analyzed wireless key extraction protocol that is demonstrably secure against passive adversaries. Our methodology uses hidden Markov models as the channel model and a dynamic programming approach to approximate conditional min-entropy but other possible instantiations of the methodology can be motivated by our work.

==> analysis-assumptions.tex <==

\appendix{Justification of Channel Assumptions}
\label{subsec:channel-assumptions}

We now argue that all channel assumptions stated in
Section~\ref{sec:learning} hold true  based on the
analysis of the experimental data collected in the test environment
described in Section~\ref{subsec:experiment-setup}.

\medskip
\noindent{\bf Stationary Memoryless Markov Process Assumption:} We
split assumption~\ref{assumption:markov} to three sub-assumptions.
Let us begin with the assumption that every channel measurement
$X_i$ depends only on the previous measurement $X_{i-1}$ for all
$i$. As mentioned in our description of our test platform, we used
an artificial delay of 1300ms between ping frames in order to induce
independence between channel samples greater than one sample apart.
To evaluate this assumption of independence we performed the
following analysis. We selected some $i \in [1+m,N]$ uniformly at
random, where $N$ is the number of samples in a node's measurements,
and $m = 500$. We then created a $(m+1)$-length row vector as
$\{X_{i}, X_{i-1}, \ldots, X_{i-m}\}$, where $X_{i-m}$ is the
$(i-m)$-th sample from a node's channel measurements. This was
repeated 10,000 times, concatenating each of the 10,000 row vectors
together to create a $10000 \times (m+1)$ matrix $A$.

The Pearson's linear correlation coefficients of the resulting
column vectors in $A$ were then computed to find the correlation of
$X_i$ with $X_{i-k}$ for each $k \in [1,500]$. From the correlation
analysis of our experimental data, we found that there exists a
statistically significant correlation between samples $X_i$ and
$X_{i-k}$ at a significance level of $\alpha = 0.05$ for values of
$k$ up to $6$. Since we want to ensure that $X_i$ and $X_{i-k}$ are
independent for $k > 1$ for our channel assumptions to hold, we
further downsample the collected data by a factor of six in order to
induce this level of independence (i.e., ensuring at least 7800ms
between samples). The remainder of our experimental analysis is
performed on this downsampled data. The correlation among signals
under downsampled data is shown in Figure~\ref{fig:downsample}.
\begin{figure}
    \centering
    \includegraphics[width=3in, height=1.5in]{downsampled-correlation.eps}
    %\resizebox{3.25in}{!}{\includegraphics{node-layout}}
    \caption{Correlation among signals in the downsampled data}
    \label{fig:downsample}
\end{figure}

%2. Take every $X_i$ as different random variable, they follow
%the identical distribution
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%
!!!!!!!!!!!!!!\emph{keep justification for $X_i$ follow identical
distribution} }%%%%%%%%%%%%%%%%%%%%%%

Next, we show that if we treat every $X_i$ as a different random
variable, they each follow an identical distribution. For this
evaluation, we employ the two-sample Kolmogorov-Smirnov (K-S) test
which accepts as input two input vectors $\vec{x}_1$ and $\vec{x}_2$
and evaluates the null hypothesis that $\vec{x}_1$ and $\vec{x}_2$
are from the same distribution against the alternative hypothesis
that $\vec{x}_1$ and $\vec{x}_2$ are from different distributions.
We randomly partitioned each node's set of channel measurements $X$
into two non-overlapping vectors $\vec{x}_1$ and $\vec{x}_2$, each
of length $|\vec{x}_1| = |\vec{x}_2| = \lfloor N/2 \rfloor$ where $N
= |X|$ is the total number of channel measurements. We then
performed a two-sample K-S test on $\vec{x}_1$ and $\vec{x}_2$ again
using a significance level of $\alpha = 0.05$. This process was
repeated 10,000 times each for Alice's and Bob's measurements (i.e.,
a total of 20,000 trials). Of those 20,000 trials, we had to reject
the null hypothesis that $\vec{x}_1$ and $\vec{x}_2$ are identically
distributed in $0.54\%$ of the trials. While we did reject the null
hypothesis in a non-zero percentage of trials, the results still
lend strong support  to the assumption that each node's channel
samples $X_i$ are identically distributed throughout each
experiment.

\ignore{%%%%%%%%%%%%%%%%%%%%
The same correlation analysis after downsampling the data is shown in
Figure~\ref{fig:sample-correlation}(b). From those results we can conclude
that, in our test environment, the assumption that samples $X_i$ and $X_{i-
k}$ are statistically independent holds true when $k > 1$ and the separation
between $X_i$ and $X_{i \pm 1}$ is greater than 7.8 seconds.

[!!!!!!! AK : \emph{ here we should argue that assumption 1(b)
holds; what is stated is different but we may keep it as a warm
up.}] }%%%%%%%%%%%%%%%%%%%%%%

Finally, we consider the assumption that the Markov process
transition probability is stationary. That is, we want to show that
the equality: $\Pr[X_i = x_1|X_{i-1} = x_0] = \Pr[X_j = x_1 |
X_{j-1} = x_0],$ holds for any $i$ and $j$ with $i \neq j$. We
randomly selected some $i$ and $j$ in $[1,N-1]$ uniformly at random
and append the channel sample $X_{i+1}$ to a vector $\vec{x}_1$ and
$X_{j+1}$ to a vector $\vec{x}_2$. This was repeated 10,000 times to
create two 10,000-element vectors. We then applied the two-sample
K-S test to $\vec{x}_1$ and $\vec{x}_2$ to determine whether the
sample distributions are identical. We found that in every test case
the resulting distributions are identically distributed at a
confidence level of $\alpha = 0.05$.

\medskip
\noindent{\bf Stationary Observation Probability Assumption:} Next,
we consider our assumption~\ref{assumption:stationary-transit} that
the channel sample observation probability is stationary.
Specifically, we want to show that $\Pr[Y_i = y | X_i = x] = \Pr[Y_j
= y | X_j = x]$ holds true for any two sample indices $i$ and $j$
with $i \neq j$, where $x$ and $y$ indicate concrete RSSI values
observed by Alice and Eve, respectively. We can easily find the
correlation between $Y_i$ and $X_{i}$ for $k \in [-500,500]$ for
each Eve node using the same approach based on computing the linear
Pearson's correlation coefficient that we described above for
evaluating the first assumption. The results were averaged across
all five eavesdropper nodes. We found that an eavesdropper
measurement $Y_i$ was statistically independent from some sample
$X_j$ collected by Alice for $i\neq j$ at a significance level of
$\alpha = 0.05$.

We use a technique similar to those above to evaluate whether
$\Pr[Y_i | X_i] = \Pr[Y_j | X_j]$ for any two sample indices $i$ and
$j$ with $i \neq j$). We first partition the set of sample indices
$I = \{1,2,\ldots,N\}$ into two equal-sized random subsets
$I^\prime_1$ and $I^\prime_2$ such that $|I^\prime_1| = |I^\prime_2|
= \lfloor N/2 \rfloor$. Eve's channel measurement set $Y$ was
similarly partitioned into two subsets $Y^\prime_1$ and
$Y^\prime_2$, such that $Y^\prime_1$ contains the measurements in
$Y$ corresponding to the channel sample indices in $I^\prime_1$ and
$Y^\prime_2$ contains the measurements in $Y$ corresponding to the
channel sample indices in $I^\prime_2$. Alice's channel measurements
were partitioned into two subsets $X^\prime_1$ and $X^\prime_2$ in
the same manner. We then compute the joint distributions between
$X^\prime_1$ and $Y^\prime_1$, as well as between $X^\prime_2$ and
$Y^\prime_2$. For each RSSI value $x \in [-24,0]$ (the range of
possible RSSI values in our experimental platform), we use a
two-sample K-S test to determine whether the two distributions
$\Pr[Y^\prime_1|X^\prime_1 = x]$ and $\Pr[Y^\prime_2|X^\prime_2 =
x]$ are identical. This process was repeated a total of 10,000 times
for each of the five eavesdropper sets $Y$ (i.e., a total of 50,000
trials). Out of the 50,000 trials, we accepted the null hypothesis
that the two distributions were identical 100\% of the time with a
significance level of $\alpha = 0.05$ and so we conclude that the
assumption $\Pr[Y_i|X_i] = \Pr[Y_j|X_j]$ holds true when $i \neq j$.

\medskip
\noindent{\bf Independent Observation Assumption:} This statement
says that the dependency that potentially exists between the
adversary's measurements comes strictly from the existing dependency
of the corresponding measurements of Alice and not any other source.
Note that  from the stationary observation probability assumption,
each $Y_i$ follows a distribution that depends only on the value of
$X_i$ and this dependency does not change over time.
This suggests that there exists a probabilistic function $F$ over
$X_i$ which can simulate the observations of Eve, i.e.,
$Y_{i}=F(X_{i})$. In such case we prove the independent
observation assumption as follows:
\[
\begin{aligned}
&Pr[Y_{1}=y_{1},\ldots,Y_{n}=y_{n}|x_{1},\ldots,x_{n}]\\
=&Pr[F(X_{1})=y_{1},\ldots,F(X_{n})=y_{n}|x_1,\ldots,x_n]\\
=&Pr[F(x_{1})=y_{1},\ldots,F(x_{n})=y_{n}]\\
=&\prod_{i=1}^{n}Pr[F(x_{i})=y_i]=\prod_{i=1}^{n}Pr[F(X_{i})=y_{i}|X_{i}=x_{i}]\\
=&\prod_{i=1}^{n}Pr[Y_{i}=y_i|X_i=x_{i}]
\end{aligned}
\]

%\medskip
\noindent{\bf Stable Conditional Min-Entropy Assumption}: The
intuition for assumption~\ref{assumption:stationary-entropy} is that
even though at some location, some observations may have better
advantage to predict the original measurement, the sequence would be
long enough, and thus when averaging across the whole sequence, the
advantage will diminish. To experimentally justify this assumption,
we calculate the min-entropy of the sequence received by node1
conditioned on node4's observation in each experiment (represented
by each 100-sample block). We observe that it is stably distributed
as shown in figure~\ref{figure:stable-entropy}.
\begin{figure}
    \centering
    \includegraphics[width=3in,height=2in]{entropy4.eps}
    %\resizebox{3.25in}{!}{\includegraphics{node-layout}}
    \caption{Distribution of conditional min-entropy in node4, x-axis is the index of
    experiment, y-axis is the value of conditional min-entropy,
    300 is the maximum entropy contained in the 100 samples}
    \label{figure:stable-entropy}
\end{figure}

%Thus  assumption \ref{assumption:independent-observation} is  justified.


==> security.tex <==
\noindent{\bf Security Arguments for Key Extraction} Next, we will
demonstrate the complete argument for the security of the three-step
key extraction protocol described above.

First, we run a number of experiments, collect enough data samples
to approximate the conditional min-entropy contained in the
measurements of Alice before bit quantization using the learning
algorithm we proposed in section~\ref{sec:learning}.

Subsequently, the security analysis should take into account the
entropy loss that occurs as follows:
%\begin{itemize}

-- Entropy loss due to quantization. In case an injective embedding
is used there will be no entropy loss in this step. Nevertheless in
any other case a significant entropy loss may occur and this should
be subtracted from $H$.

-- Entropy loss due to message passing. In order for Alice and Bob
to achieve information reconciliation and privacy amplification,
they need to exchange a number of messages that depend on their
measurements(also in the bit quantization step in some of the
previous works). A worst case information-theoretic approach would
calculate the amount of entropy that can leak in these messages and
then subtract it from $H$.
%\end{itemize}

Naturally, if the value $H$ becomes 0 due to the above steps then
there is no entropy left and it is plausible that the adversary can
break the protocol and recover the key given its view. In the other
case if $H>0$ and there is enough uncertainty left which can be
extracted in the form of a uniformly distributed key in a privacy
amplification step (and recall that for this step a  randomness
extractor is employed by our protocol).

Last, we will identify and justify all the assumptions made from
experimental data.

With the above security argument framework, we could properly
determine the concrete parameters of the key extraction protocol
from a set of experiments so that a strong security guarantee of the
extracted key is provided.


\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%sum to estimate average case conditional entropy
It follows that if we have the parameters of the HMM that expresses
the measurements of Alice and Eve over the channel, then we can use
the Viterbi algorithm to estimate the conditional min-entropy of
Alice's measurements as follows. We first perform a series of $M$
experiments each one with $N$ measurements each. For each one, say
the $j$-th experiment, we record the measurements of Eve, and we use
them together with the HMM parameters to calculate the conditional
max probability as $P^*_j = \max_{s}\delta_{n}(s)$. Finally we
estimate the conditional min-entropy as $H^* = -\log ( \sum_{j=1}^M
P^*_j)$.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%From the way we defined the  quantization algorithm, we can see that, each $B_i$ is fully
%determined by the sequence of values
%$X_{i-m+1},\ldots ,X_{i}$. Let $S_1$ be the set containing all sequences of
%$X_{i-m+1},..,X_{i}$ values that after the thresholding step they become $LH\ldots H$ or
%$MH\ldots H$, and let $S_0$ contain all sequences that become
%$HL\ldots L$ or $ML\ldots L$
%after the thresholding step. We   can write $B_i$ as a deterministic function
%of these values as follows:
%$$
%B_i=f(X_{i-m+1},..,X_i)=\left\{
%\begin{aligned}
%&1, if\hspace{1mm} X_{i-m+1},..,X_i\in S_1\\
%&0, if\hspace{1mm} X_{i-m+1},..,X_i\in S_0\\
%&?, otherwise
%\end{aligned}
%\right.
%$$
%
%
%Based on the above we  consider the joint distribution
%%
%\[ Pr[B_1\ldots B_n \mid Y, E]  \]
%
%where $Y$ is the signal  obtained by the  eavesdropper and
%$E$ is the string that reveals the excursion points.
%
%
%Directly applying Bayesian formula, we have:
%$$
%\begin{aligned}
%&Pr[B_1,..,B_N|Y,E]&\\
%=&\prod_{i}Pr[B_i|B_{i-1},..,B_1,Y,E]&\\
%=& \prod_{i:e_i=1} Pr[B_i | B_{j}, \mbox{ for } j <i :  e_j =1, Y, E]  &
%\end{aligned}
%$$
%To simplify the formula, we need the following assumptions for channel measurements which will be justified later.
%
%%$X_1,..,X_m$, and $Y_1,..,Y_m$ are random variables represent
%%channel measurements of Alice and raw data of observations for ping data of Eve
%%respectively, our main assumptions which will be justified later are as follows:
%\begin{itemize}
%\item[1.] For $i,j$ with $|i-j|> k$, $X_i,X_j$ are independent.
%\label{assumption:independent}
%\item[2.] All the $X_i$ as distinct random variables,  follow the
%same probability distribution. \label{assumption:indentical distribution}
%\item[3.] For every $i$, $Y_i$ only depends on $X_i$, and for any $i,j$, we have $Pr[Y_i|X_i]=Pr[Y_j|X_j]$.
%\label{assumption:independent observation}
%\end{itemize}
%
%With these three, it is reasonable to further assume the conditional independence for
%message blocks, that is:
%\begin{itemize}
%\item[4.] For any $i$, $X_{i-m+1},..X_i$ is independent of $$(X_{i-2m-1},..X_1,Y_1,..,Y_{i-m-k},Y_{i+k+1}..Y_n)$$
%given $X_{i-2m},..,X_{i-m-1},Y_{i-m-k+1},..,Y_{i+k}$, that is
%\label{assumption:conditional independence}
%$$
%\begin{aligned}
%&Pr[X_{i-m},..X_{i}|X_{i-m-1},..X_{1},Y_1,..,Y_n]\\
%&=Pr[X_{i-m+1},..X_{i}|X_{i-m-k+1},..,X_{i-m},Y_{i-m-k+1},..Y_{i+k}].
%\end{aligned}
%$$
%and also $X_{i-m+1},..X_i$ is independent of $$(X_{i-2m-1},..X_1,Y_1,..,Y_{i-m-k},Y_{i+k+1}..Y_n)$$ given $Y_{i-m-k+1},..,Y_{i+k}$.
%
%\item[5.] For any $i,t,j$, $$Pr[X_{i},..X_{i+t}|Y_{i},..Y_{i+t}]=Pr[X_{j},..X_{j+t}|Y_{j},..Y_{j+t}]$$.
%\end{itemize}
%
%For assumption 4, for simple case, when $m=1$, given $Y_{i-1},Y_i,Y_{i+1}$ or $X_{i-2},Y_{i-1},Y_i,Y_{i+1}$,
% $X_i$ is independent of $(X_i-2,..X_1, Y_1,..Y_i-2,Y_i+2,..Y_n)$.
%
%\begin{definition}
%For $e_i=e_j=1$, with $|i-j|\leq max(m,k)$, then $B_i, B_j$ are correlated, we call
%this kind of pair tight pair, and further, $S^{*}=\{i\in [1,N]|e_i=1, \forall j<i, B_i, B_j \hspace{1mm}are\hspace{1mm}not\hspace{1mm}tight\}$,
%and $T_i=\{j\in[1,N]|j<i,B_i, B_j \hspace{1mm}are\hspace{1mm} tight\}$.
%\end{definition}
%
%From Figure~\ref{fig:relation}, we can see that, for any $|i-j|>max(m,k)$,
%and $e_i=e_j=1$, due to the property of our excursion algorithm, all
%the values which fully decide $B_i, B_j$ have no intersection, so
%such $B_i,B_j$ are independent. The only correlated $B_i, B_j$ is
%the ones with $|i-j|\leq max(m,k)$.
%
%\begin{claim}
%If assumption~\ref{assumption:independent} and assumption~\ref{assumption:conditional independence} hold, we could derive:
%
%\hspace{1cm} $Pr[B_i|B_{i-1},..,B_1,Y,E]$
%$$
%=\left\{
%\begin{aligned}
%&Pr[B_i|Y_{i-m-k+1},..,Y_{i+k}],  i\in S^{*}.\\
%&Pr[B_i|B_{j_1},..,B_{j_s},Y_{i-m-k+1},..,Y_{i+k}], \{j_1,..j_s\}=T_i
%\end{aligned}
%\right.
%$$
%\end{claim}
%
%\begin{proof}
%$B_i$ is a deterministic function of $X_{i-m+1},..X_{i}$,
%and by reading the excursion points, the condition becomes either case of assumption~\ref{assumption:conditional independence},
%so only correlated parts are left.
%\end{proof}
%
%Next, we want approximate such conditional probability from real experiments. The following claim assures
%the index does not influence the estimation.
%
%\begin{claim}
%\label{claim:consistency}
%
%We would derive from our channel assumption that for any $i,j\in E$,
%we have $Pr[B_i=b|B_{i-1},..,B_1,Y,E]=Pr[B_j=b|B_{j-1},..,B_1,Y,E]$.
%\end{claim}
%
%\begin{proof}
%Since $B_i$ could be written as a deterministic function of $X_{i-m+1},..,X_i$,
%thus $B_i=b \Leftrightarrow X_{i-m+1},..,X_i\in S_b$, for the points in the excursion,
%solely $X_i$ could decide the bit.
%
%When $i, i-1$ are not tight, all previous bit of $B_i$ are
%independent of it, thus for $b=1$,
%\begin{align}
%&Pr[B_i=b|B_{i-1},..,B_1,Y,E]\notag\\
%&=Pr[B_i=b|y_{i-m-k},..,y_{i+k},E]\notag\\
%&=\sum_{x_i>q_{+}}Pr[x_i|y_{i-m-k+1},..,y_{i+k}]\notag\\
%&=\sum_{x_i>q_{+}}Pr[X_i=x_i|Y_i=y_{i}]
%\end{align}
%Because of assumption~\ref{assumption:indentical distribution} and
%assumption~\ref{assumption:independent observation}, for each
%summand of (1), we have
%$Pr[X_i=x_i|Y_i=y_{i}]=Pr[Y_i=y_i|X_i=x_i]Pr[X_i=x_i]/Pr[Y_i=y_i]$,
%while each component is the same for different $i,j$, so claim holds
%in this case. It is the same for $b=0$.
%
%When previous bit correlated with $B_i$,
%$Pr[B_i|B_{i-1},y_{i-m-k},..,y_{i+k}]=Pr[B_i,B_i-1|y_{i-m-k},..,y_{i+k}]/Pr[B_{i-1}|y_{i-m-k},..,y_{i+k}]$,
%the denominator is the same, thus we only need to show for the upper part:
%When $b=b_1=1$,
%\begin{align}
%&Pr[B_i=b,B_{i-1}=b_{1}|y_{i-m-k},..,y_{i+k},E]\notag\\
%&=\sum_{x_i>q_{+},x_{i-1}>q_{+}}Pr[x_i,x_{i-1}|y_{i-m-k+1},..,y_{i+k}]\notag\\
%&=\sum_{x_i>q_{+},x_{i-1}>q_{+}}Pr[X_i=x_i,X_{i-1}=x_{i-1}|Y_i=y_{i},Y_{i-1}=y_{i-1}]\notag
%\end{align}
%From assumption 5, it is obvious that the claim holds. And it is similar for all other $b,b_1$, and the case several more previous bits correlated with $B_i$.
%\end{proof}
%
%With claim ~\ref{claim:consistency}, we could estimate each
%component of conditional probability by counting throughout all
%samples.
%
%We create a table from experiment data for all $y$-sequence with
%length $2k+m+1$ appeared, and count the number of occurrence for
%each sequence throughout all samples. Then the following columns are
%arranged as follows,
%
%The second column is labeled as $n_0$, and composed of number of
%appearance of each $y$-sequence together with the corresponding
%$B_i$ to be $0$.
%
%The third column is labeled as $n_1$,the number of appearance of
%each $y$-sequence together with the corresponding $B_i=1$.
%
%The fourth column is labeled as $n_{00}$, the number of appearance
%of each $y$-sequence together with the corresponding $B_i=0$ and the
%previous bit of key is $0$.
%
%The fifty column is labeled as $n_{01}$, the number of appearance of
%each $y$-sequence together with the corresponding $B_i=1$ and the
%previous bit of key is $0$.
%
%For each row, (a $y$-sequence), go on with this procedure for the columns until
%collect all possible values for joint appearance of all correlated previous bits.
%Normally, number of previous bits correlated to each bit of
%key is small, we could prepare all those numbers in a table. If this
%is too big, we can simply drop some correlated bits to make it into two smaller set, during the bit
%quantization step by reducing the excursion points. Or ignore those
%component, just set the value to be 1 for $Pr[B_i|B_i-1,..,B_1,Y]$
%which has too many $B_j$ in the condition.
%
%Then, for each bit of the key material, if for $i$, $B_i$ does not correlate with its neighbor, then,
%$Pr[B_i=b|B_i-1,..B_1,Y]=Pr[B_i=b|Y_{i-m-k+1}=y_{i-m-k+1},..,Y_{i+k}=y_{i+k}]$,
%we search the corresponding sequence $y_{i-m-k+1},..,y_{i+k}$, and set
%$n_b/(n_0+n_1)$ as the estimation for this probability, and pick the bigger one as the value of this component.
%
%In other cases, $B_i$ has correlated previous bits, say only
%$B_{i-1}$, that is
%$Pr[B_i=1|B_i-1,..B_1,Y]=Pr[B_i=1|B_{i-1}=b,Y_{i-m-k+1}=y_{i-m-k+1},..,Y_{i+k}=y_{i+k}]$,
%then we search for the $y$-sequence, and set $n_{b1}/n_{b1}+n_{b0}$
%as the estimation for this value. similar for more bit correlated.
%%AK : GAP HERE GAP HERE
%%
%%
%%which eventually concludes that it is equal to
%%
%%\[ =  \prod_i Pr[B_i | B_j \mbox{ for max } j<i, Y_{i-m-k+1}, \ldots, Y_{i+k} ] \]
%
%
%
%Recall that, we need to calculate for any given $\bar{y}=y_1,\ldots,y_N$,and $\bar{e}=e_1,\ldots,e_N$,
%$$
%\begin{aligned}
%&H_\infty(B|Y=\bar{y},E=\bar{e})&\\
%&=-\log \max_{\bar{b}}
%Pr[B=\bar{b}|Y=\bar{y},E=\bar{e}]&\\
%&=-\log
%\max_{b_1,..,b_n}Pr[B_1,..,B_n=b_1,..,b_n|Y=\bar{y},E=\bar{e}]&
%\end{aligned}
%$$
%
%For the chain of bits correlated with neighbor, and the chain length is no more than 20, we do the brute-force algorithm to
%get the maximum value for the block $$Pr[B_i|\bar{Y}]Pr[B_{i+1}|B_i,\bar{Y}]..Pr[B_{i+t}|B_{i+t-1}..,B_i,\bar{Y}]$$.
%
%Then we multiply all the maximum probability for every block to get the estimation for the product.
%
%There are some other issue to consider when doing entropy
%estimation. One is package loss for Eve. From security point of
%view, if entropy is high enough even if we give eavesdropper the
%best advantage, then in general, system would be secure. So we only
%consider the package that Alice, Bob and Eve all receive when doing
%security analysis.
%
%Since the range for signal strength value is [-128,128], when the
%$y$-sequence we used to create the the table is long, we will need
%enormous data with exponential size to do the counting. While, when
%all nodes parse the signal, the least significant bits would not
%play important role in deciding the signal, so we could reduce
%precision for the sample values to approximate the real one, just by
%dropping some least significant bits of the sample value.
%
%To compute the average-case min-entropy, according to the
%definition, we need to get expected value. We can merge all the
%experiments data, and then cut into shorter pieces, each piece is
%counted as one experiment. We will have different $\bar{y},\bar{e}$
%for each experiment. Then we compute the product of all the
%conditional probability as above, and then apply logarithm to the
%average of them.
%%Now using the above we have
%%
%%AK : GAP HERE GAP HERE
%%
%%
%%AK : THE REST OF SECTION USE AS NEEDED.
%
%
%
%%\begin{claim}
%%\label{claim:estimate} Let $Y=Y_1,..,Y_n$, and $E={e_1,..,e_n}$
%%represent the excursions, where $e_i=1$ if $i$ is an excursion
%%point, and $e_i=0$ otherwise. This is essentially the same as the
%%set of excursion points. $\rho_A$ is key of Alice, $d$ is the
%%Hamming distance between Alice and Bob's key. Then, based on the
%%assumptions above, we can estimate the average min-entropy of key
%%material conditioned on all Eve sees by estimating simple
%%conditional probabilities as follows.
%%\end{claim}
%
%
%
%
%%We first simplify the formula of the conditional min-entropy by eliminating the
%%unrelated variables in conditions, and then estimate all the
%%probabilities from experimental data.
%%
%%\textbf{Simplify the formula:}
%%We use a new way to represent the excursions $E$ Alice and Bob have in common,
%%instead of list all the positions, we set $E=e_1,\ldots,e_N$, and $e_i=1$, if $i$ is an
%%excursion point, and $e_i=0$ if $i$ is not excursion. This representation and list of
%%all excursion points are obviously the same.
%%
%%For any given $\bar{y}=y_1,\ldots,y_N$,and $\bar{e}=e_1,\ldots,e_N$,
%%$$
%%\begin{aligned}
%%&H_\infty(B|Y=\bar{y},E=\bar{e})&\\
%%&=-\log \max_{\bar{b}}
%%Pr[B=\bar{b}|Y=\bar{y},E=\bar{e}]&\\
%%&=-\log
%%\max_{b_1,..,b_n}Pr[B_1,..,B_n=b_1,..,b_n|Y=\bar{y},E=\bar{e}]&
%%\end{aligned}
%%$$
%%
%%For any $B_i$, it is totally decided by $m$ values
%%$X_{i-m+1},..,X_{i}$, so to any $j$ with $j<i-m-k+1$ or $j>i+k$, $Y_j$ is
%%independent with all those $m$ values, then we have:
%%
%%$$
%%\begin{aligned}
%%&Pr[B_i|Y_j]&\\
%%&=\sum_{X_{i-m+1},..,X_i}Pr[B_i|Y_j,X_{i-m+1},..,X_i]Pr[X_{i-m+1},..,X_i]&\\
%%&=\sum_{X_{i-m+1},..,X_i}Pr[B_i|X_{i-m+1},..,X_i]Pr[X_{i-m+1},..,X_i]&\\
%%&=Pr[B_i]&
%%\end{aligned}
%%$$
%%This means $B_i$ is independent of any such $Y_j$, the only $Y$
%%values related to $B_i$ are $Y_{i-m-k+1},..,Y_{i+k}$.
%%
%%Since from excursions $E$, Eve knows exactly the non-excursion
%%points, so $B_i$ in non-excursion position $i$ has no uncertainty
%%there.
%%
%%, and $e_i=e_j=1$, we called this kind of
%%excursion pairs tight excursions. Definition as follows:
%
%
%%$abcd\fbox{ef}gh$
%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[xshift=50pt]
%
%\draw (-1,0) node {$Y_1,..,Y_{i-m}$,};
%\draw (5.3,0) node {$Y_{j+1},..,Y_n$};
%\draw (1,0) node {$Y_{i-m+1},..,Y_i$,};
%\draw (3.4,0) node {$Y_{j-m+1},..,Y_j$,};
%
%\draw (-1,-1) node {$X_1,..,X_{i-m}$,};
%\draw (5.3,-1) node {$X_{j+1},..,X_n$};
%\draw (0,-1.2) rectangle (2.1,-0.8);
%\draw (2.2,-1) node {...};
%\draw[style=dashed] (2.55,-1) ellipse (30pt and 10pt);
%\draw (2.4,-1.2) rectangle (4.5,-0.8);
%\draw (1,-1) node {$X_{i-m+1},..,X_i$,};
%\draw (3.4,-1) node {$X_{j-m+1},..,X_j$,};
%
%\draw (-1,-2) node {$B_1,..,B_{i-m}$,};
%\draw (5.3,-2) node {$B_{j+1},..,B_n$};
%\draw (1,-2) node {$B_{i-m+1},..,B_i$};
%\draw (3.4,-2) node {$B_{j-m+1},..,B_j$};
%
%\draw (1.9,-0.3) -- (1.9,-0.8);
%\draw (4.3,-0.3) -- (4.3,-0.8);
%\draw (0.1,-0.3) -- (0.1,-0.8);
%\draw (2.5,-0.3) -- (2.5,-0.8);
%
%\draw (1.9,-1.3) -- (1.9,-1.8);
%\draw (1.0,-1.3) -- (1.9,-1.8);
%\draw (0.1,-1.3) -- (1.9,-1.8);
%\draw (4.3,-1.3) -- (4.3,-1.8);
%\draw (3.5,-1.3) -- (4.3,-1.8);
%\draw (2.5,-1.3) -- (4.3,-1.8);
%\end{tikzpicture}
%\caption{\label{fig:relation}Relationship between measurement and key material when $m\geq k$}
%\end{center}
%\end{figure}
%
%
%%?????
%
%
%
%
%
%%
%%\textbf{Estimation from experimental data}
%
%
%%$$
%%\begin{aligned}
%%&Pr[B_i=b|y_{i-m-k},..,y_{i+k}]\\
%%=&\sum_{x_{i-m+1,..,x_i}\in S_b}
%%Pr[x_{i-m+1},..x_i|y_{i-m-k},..,y_{i+k}]\\
%%\end{aligned}
%%$$
%%For each component, similar to the simplification in last part,
%%$$
%%\begin{aligned}
%%&Pr[x_{i-m+1},..x_i|y_{i-m-k},..,y_{i+k}]\\
%%=&\prod_{t}Pr[X_t=x_t|X_{t-1}=x_{t-1},..,X_{t-k}=x_{t-k},Y_t=y_{t}]\\
%%\end{aligned}
%%$$
%%We further take out each component of this formula,
%%%
%%\begin{align}
%%&Pr[X_t=x_t|X_{t-1}=x_{t-1},Y_t=y_{t-1}]\notag\\
%%&=\frac{Pr[X_t=x_t,X_{t-1}=x_{t-1},Y_t=y_t]}{Pr[X_{t-1}=x_{t-1},Y_t=y_t]}\notag\\
%%&=\frac{Pr[X_{t-1}=x_{t-1},Y_t=y_t|X_t=x_t]Pr[X_t=x_t]}{Pr[X_{t-1}=x_{t-1}]Pr[Y_t=y_t]}\\
%%&=\frac{Pr[X_{t-1}=x_{t-1}|X_t=x_t]Pr[Y_t=y_t|X_t=x_t]}{Pr[Y_t=y_t]}
%%\end{align}
%
%%(1) is because of the independence of $X_{t-1}$ and $Y_t$. We have
%%$Pr[X_t]=Pr[X_s]$, $Pr[X_t|X_{t-1}]=Pr[X_s|X_{s-1}]$, and
%%$Pr[Y_t|X_t]=Pr[Y_s|X_s]$, then
%%$Pr[Y_t]=\sum_{x}Pr[Y_t|X_t=x]Pr[X_t=x]=\sum_{x}Pr[Y_s|X_s=x]Pr[X_s=x]=Pr[Y_s]$.
%%Having all these, now substituting $t$ to any $s$, all components in
%%(2) are the same, thus every component in the product is the same.
%%Tracing back further, any component in the sum is the same, so we
%%get, for any $i,j$,
%%$Pr[B_i|y_{i-m+1},..,y_{i}]=Pr[B_j|y_{j-m+1},..,y_{j+1}]$, which is
%%the statement of our claim.
%
%%
%
%
%
%
%%We repeat experiments in the same setting for several times, say 30 times.
%%
%%In each experiment, we could get a key material $B_1,..,B_N$, a sequence of eavesdropper's
%%observations $\bar{y}$ and excursion points $\bar{e}$.
%%We create a table, and list all the time of appearances of $y_{i-m-k+1},..,y_{i+k}$ with length $2k+m$ in all
%%those experiments, and correspondingly, the time of 0s for the $B_i$. Then we compute
%%the conditional probability $max Pr[B_1,.,B_N|\bar{y},\bar{e}]$ for each experiment as follows:
%%
%%For every $i$, that $e_i=e_j=1$, and $j$
%%is the previous excursion of $i$, we check whether $|i-j|>max(k,m)$, if yes, $B_i, B_j$ is not tight, and
%%$i$ is in $S^*$. We find the sequence of $m$
%%consecutive values $y_{i-m-k+1},..,y_{i+k}$ from Eve's observations for this location.
%%We then check the table, compute $Pr[B_i=0|y_{i-m-k+1},..,y_{i+k}]$ by dividing the two numbers of appearance in
%%the table, if it is larger than 1/2, set $Pr[B_i|y_{i-m-k+1},..,y_{i+k}]$ equal to that value, or set it equal to 1-$Pr[B_i=0|y_{i-m-k+1},..,y_{i+k}]$.
%%Since some sequences appear very infrequently, we only consider only the sequences that appear more than $t$
%%times, we ignore those scarce sequence appeared less than $t$ times, and  simply set the corresponding probability $Pr[B_i|y_{i-m-k+1},..,y_{i+k}]$ to be 1.
%%
%%For $i$ with $e_i=1$ and $B_j$ at its previous excursion is tight
%%with $B_i$, since those tight pairs appear infrequently, we simply set
%%the corresponding conditional probability to be 1. (Or we can do brute
%%force search for the maximal value for products of conditional
%%probabilities of such pairs to improve the estimation. Ignoring such
%%pairs does not influence the security analysis, since we would get higher
%%entropy if we have a better estimation of those conditional probabilities.)
%%
%%Then we multiply all the values of each component to get an estimation of $max Pr[B_1,.,B_N|\bar{y},\bar{e}]$.
%%
%%Then repeat the procedure of doing estimations for all those experiments with different $\bar{y},\bar{e}$, and make an
%%average of the conditional probabilities, and then apply the logarithm.
%
%Combine the two claims and estimation above, we summarize the
%estimation procedure:
%\begin{claim}
%Based the three assumptions of channel properties, we could get an estimation
%of average case min-entropy based on all eavesdropper sees
%\begin{align}
%&\widetilde{H}_\infty(B|Y,E)\notag\\
%=&-\log E_{\bar{y},\bar{e}}(\max_{b_1,..b_N}Pr[B_1,..,B_N|Y=\bar{y},E=\bar{e}])\notag
%\end{align}
%in following steps:
%\begin{enumerate}
%\item{} Intersect the samples of Alice, Bob and Eve according to the
%sample sequence number.
%\item{} Sometimes, if $k$ too big, which means the correlation among
%raw measurements last too long, we could further drop data, like
%picking 1 out of $k/2+1$.
%\item{} Reducing measurements precision for all data if needed by
%doing right shift.
%\item{} Run bit quantization algorithm to generate key material and
%excursion, drop bits to make consecutive substring in the key
%material shorter if necessary.
%\item{} Create table as described above according to the generated
%key material.
%\item{} Cut the key material into several pieces, estimate conditional probability as described above, and
%multiply all components, then averaging all the probabilities, and
%apply logarithm to return the approximated average-case min-entropy
%during the bit quantization phase.
%\end{enumerate}
%%by $-\log E_{\bar{y},\bar{e}}(\max_{b_1,..b_N}\prod_{i\in S^{*}}Pr[B_i|Y_{i-m-k+1},..,Y_{i+k}])$.
%\end{claim}

